Deep Learning-based Cooperative LiDAR Sensing for Improved Vehicle Positioning

Accurate positioning is known to be a fundamental requirement for the deployment of Connected Automated Vehicles (CAVs). To meet this need, a new emerging trend is represented by cooperative methods where vehicles fuse information coming from navigation and imaging sensors via Vehicle-to-Everything (V2X) communications for joint positioning and environmental perception. In line with this trend, this paper proposes a novel data-driven cooperative sensing framework, termed Cooperative LiDAR Sensing with Message Passing Neural Network (CLS-MPNN), where spatially-distributed vehicles collaborate in perceiving the environment via LiDAR sensors. Vehicles process their LiDAR point clouds using a Deep Neural Network (DNN), namely a 3D object detector, to identify and localize possible static objects present in the driving environment. Data are then aggregated by a centralized infrastructure that performs Data Association (DA) using a Message Passing Neural Network (MPNN) and runs the Implicit Cooperative Positioning (ICP) algorithm. The proposed approach is evaluated using two realistic driving scenarios generated by a high-fidelity automated driving simulator. The results show that CLS-MPNN outperforms a conventional non-cooperative localization algorithm based on Global Navigation Satellite System (GNSS) and a state-of-the-art cooperative Simultaneous Localization and Mapping (SLAM) method while approaching the performances of an oracle system with ideal sensing and perfect association.

==> sections/Cooperative_lidar.tex <==
\section{Deep learning-based environmental perception}
\label{sec:coop_lidar_pos}

\label{subsec:coop_lidar_localization}


In this section, we detail the strategies employed for letting each vehicle perceive the driving environment. 
In particular, \ac{dl}-based 3D object detectors are used to efficiently process the LiDAR point clouds and obtain the position of the static objects present in the vehicles' surroundings. 
Given the ego-vehicle LiDAR data, the 3D object detectors provide at the output a set of $N_B$ candidate bounding boxes $B = \{1, \ldots, N_{B}\}$ physically encapsulating the detected poles. 
We assume that each box is always related to an object, i.e., we neglect any false positive, and is described as
\begin{equation}
\widehat{\mathbf{b}}_{j}= [\widehat{\mathbf{u}}_{j}^{(\text{B})}\, \widehat{\mathbf{d}}_{j}\,  \widehat{\gamma}_{j} ]^{\mathrm{T}} \, \qquad \text{with} \,  j = 1, \dots , N_{B}
\end{equation}  
where $\widehat{\mathbf{u}}_{j}^{(\text{B})}~=~ [\widehat{u}_{x,j}^{(\text{B})}\, \widehat{u}_{y,j}^{(\text{B})}\, \widehat{u}_{z,j}^{(\text{B})}]$ is the estimated object's center, $\widehat{\mathbf{d}}_{j} = [\widehat{\ell}_{j} \, \widehat{w}_{j} \, \widehat{h}_{j}]$ contains the object's dimensions, namely the length, width and height, while $\widehat{\gamma}_{j}$ is the yaw angle.

To comprehensively characterize the proposed cooperative localization framework, we employ two state-of-the-art 3D object detection methods with increasing complexity, namely PointPillars and Part-$\text{A}^2$ that are based on the single-stage and double-state paradigms, respectively.
In the following, we initially describe the inner workings of PointPillars (Sec.~\ref{subsec:pointpillars}) and then present the Part-$\text{A}^2$ method (Sec.~\ref{subsec:parta2}). 
 

\subsection{PointPillars}
\label{subsec:pointpillars}

%\textbf{PointPillars~\cite{point_pillars}:} 
PointPillars is a single-stage object detector that directly processes the input point cloud and extracts important features organized in pillars through the employment of PointNet~\cite{pointnet} modules.
The encoded features are then processed by a standard region proposal network to obtain the final predictions.
In the following, we explain its inner working principles and how the bounding boxes are obtained.


Starting from a single-vehicle point cloud $\mathbf{P} = [\mathbf{p}_{1} \cdots \mathbf{p}_{N_{\ell p}}]^{\mathrm{T}}
\triangleq \mathbf{P}_{v,t}$ \footnote{We use this abuse of notation to simplify the disclosure in this section.} of $N_{\ell p}$ points, PointPillars discretizes it into an evenly-spaced $x$-$y$ grid comprised of $\mathcal{P}$ non-empty pillars each containing exactly $N_p$ points\footnote{This is done by either randomly removing points or padding with zeros pillars exhibiting more or less than $N_p$ points, respectively.}.
After the pillars creation, each point $\mathbf{p}_{\ell} = [p_{x,\ell}, p_{y,\ell}, p_{z,\ell}]$ with $\ell = 1, \ldots, N_{\ell p}$ is decorated with additional information as follows
\begin{equation}
    \overline{\mathbf{p}}_{\ell} = [\mathbf{p}_{\ell}, r_{\ell}, \Delta p_{\ell,x}^c, \Delta p_{\ell,y}^c, \Delta p_{\ell,z}^c, \Delta p_{\ell,x}^p, \Delta p_{\ell,y}^p]^{\mathrm{T}}
    \label{eq:encoding}
\end{equation}
where $r_{\ell}$ is the scalar reflectance value associated to the point $\mathbf{p}_{\ell}$, $\Delta p_{\ell,x}^c$, $\Delta p_{\ell,y}^c$ and $\Delta p_{\ell,z}^c$ denote the x, y and z coordinates of the average of all points contained in the correspoding pillar, respectively, while $\Delta p_{\ell,x}^p$ and $\Delta p_{\ell,y}^p$ are the x and y offsets between $\mathbf{p}_{\ell}$ and the pillar center\footnote{In principle, $\Delta \mathbf{p}^{p}_{j}$ can contain also the offset with respect to the z-axis. However, PointPillars supports pillars with unlimited height in contrast to, for example, voxelization-based methods that apply a 3D discretization of the point cloud.
Thus, it is not required to define the offset for the z-axis.}.
The rationale behind this process is that, once all points $\mathbf{p}_{\ell}$ have been encoded as in \eqref{eq:encoding}, they can be aggregated into a single structure, namely a 3D tensor of dimension $9 \times \mathcal{P} \times N_p$, and can be efficiently processed by standard \acp{cnn}.
A simplified version of PointNet~\cite{pointnet}, composed by a convolutional layer followed by a batch normalization layer with ReLu activation function and a max pooling operation, is then used to transform the tensor into a $C \times \mathcal{P}$ feature map.
Finally, a pseudo-image of size $C \times H \times W$, with $C$, $H$ and $W$ denoting the number of channels, heigh and widht of the canvas, respectively, is created by scattering back the feature map to the original pillars positions.


The estimation of the 3D bounding boxes relies on a region-proposal network that directly processes the 2D pseudo-image extracted from the previous processing step. 
The region-proposal network comprises a backbone and a detection head~\cite{point_pillars}. 
The backbone is composed by a top-down and a bottom-up network.
The former is composed by three convolutional blocks and its goal is to learn features at increasingly small spatial resolutions. 
On the other hand, the latter takes as input the outputs produced by the top-down module and uses three upsampling blocks, implemented using transposed convolutional layers, to increase the resolution of the top-down features.
Then, the upsample features are concatenated together and are fed to the detection head which is responsible for generating the final bounding boxes. 
In particular, the standard \ac{ssd} head is used where prior boxes, also referred to as anchor boxes, are generated all over the features maps (according to a pre-fixed grid and bounding box dimensions) and matched to the ground-truths according to their 2D overlap.


As far as the training is concerned, PointPillars is trained by minimizing the loss presented in~\cite{point_pillars}. 
Let us suppose that $\{\mathbf{b}_{j}, \widehat{\mathbf{b}}_{j} \}$ is a pair of ground-truth and predicted bounding boxes, PointPillars aims at minimizing the following residuals
\begin{align}
\Delta b_{x} &= \dfrac{\Delta u_{b,x}}{d_{xy}} , \Delta b_{y} = \dfrac{\Delta u_{b,y}}{d_{xy}}, \Delta b_{z} = \dfrac{\Delta u_{b,z}}{h_{j}}, \Delta d_{w} = \log \dfrac{\widehat{w}_{j}}{w_{j}}, \nonumber \\
\Delta d_{\ell} &= \log \dfrac{\widehat{\ell}_{j}}{\ell_{j}}, \Delta d_{h} = \log \dfrac{\widehat{h}_{j}}{h_{j}}\, ,  
\Delta \gamma = \sin{\widehat{\gamma}_{j} - \gamma_{j}} \, ,
\end{align}
where $\Delta u_{b,x} = \widehat{u}_{x,j}^{(\text{B})} - u_{x,j}^{(\text{B})}$, $\Delta u_{b,y} = \widehat{u}_{y,j}^{(\text{B})} - u_{y,j}^{(\text{B})}$ and $\Delta u_{b,z} = \widehat{u}_{z,j}^{(\text{B})} - u_{z,j}^{(\text{B})}$, while $d_{xy} = \sqrt{w_j^{2} + h_{j}^2}$.
Then, the localization loss is evaluated as 
\begin{align}
\mathcal{L}_{loc} =&\, \mathrm{S_{L1}}(\Delta b_x) + \mathrm{S_{L1}}(\Delta b_y) + 
\mathrm{S_{L1}}(\Delta b_z) + 
\mathrm{S_{L1}}(\Delta d_w) 
\nonumber \\ &+ 
\mathrm{S_{L1}}(\Delta d_{\ell}) + 
\mathrm{S_{L1}}(\Delta d_h) +
\mathrm{S_{L1}}(\Delta \gamma) \, ,
\label{eq:loc_loss_pointpillars}
%&+
%\mathrm{Sm_{L1}}(\Delta \gamma)
%\sum_{g \in (b_x, b_y, b_z, d_{w}, d_{\ell}, d_{h}, \gamma)} \mathrm{Smooth_{L1}}(\Delta g)
\end{align}
where $\mathrm{S_{L1}}(.)$ is the smooth L1 loss~\cite{smooth_l1} 
\begin{equation}
\mathrm{S_{L1}}(x) = 
\begin{cases}
0.5 x^2    &  \mathrm{if} |x| < 1 \, , \\
|x| - 0.5    & \mathrm{otherwise} \, .
\end{cases}
\end{equation}
To overcome the inability of the localization loss to distinguish flipped boxes, an additional softmax direction loss $\mathcal{L}_{dir}$ is used to classify the bounding box direction over discretized angles, as performed in ~\cite{point_pillars}.
On the other hand, the focal loss is used as classification loss due to the large imbalance between ground-truth and prior boxes, and is computed as 
\begin{equation}
\mathcal{L}_{cls} = -\alpha (1 - p)^{\nu} \log p \, ,
\label{eq:focal_loss}
\end{equation}
where $p$ is the class probability of an anchor, $\alpha = 0.25$ and $\nu = 0.2$.
Combining all aforementioned loss terms, the PointPillars trainable weights are updated by minimizing the following loss
\begin{equation}
\mathcal{L}_{tot} = \dfrac{1}{N_{pos}} (\beta_{loc} \mathcal{L}_{loc} + \beta_{cls} \mathcal{L}_{cls} +  \beta_{dir} \mathcal{L}_{dir}) \, ,
\end{equation}
where $N_{pos}$ is the number of positive anchors, which are predicted bounding boxes that have the highest matching with respect to the ground-truth bounding boxes or have a matching score greater than a threshold, while $\beta_{loc} = 2$, $\beta_{cls}= 1$ and $\beta_{dir} = 0.2$ as in the original implementation~\cite{point_pillars}.

\subsection{Part-$A^{2}$}
\label{subsec:parta2}

{Part-$A^{2}$ is a double-stage 3D object detector that introduces the concept of intra-object part estimation and aggregation.
It extends the PointRCNN architecture~\cite{point_rcnn} to concurrently learn segmentation masks for discerning foreground points, classify their position inside the bounding box and generate 3D proposals, i.e., rough bounding box estimates.
The proposal are then fed to a part-aggregation network that is responsible for generating the final predictions, exploiting also the intra-object part information produced in the preceding stage. 
Note that we use in our experiments the Part-$\text{A}^2$-Anchor, which uses prior boxes for the proposal generation process. 
In the following, we briefly describe the overall architecture and how the bounding boxes are estimated.


In contrast to PointPillars, given the single-vehicle point cloud $\mathbf{P}
$, Part-$\text{A}^2$ process it using voxelization. 
In particular, a regular 3D grid is computed starting from $\mathbf{P}$ and the points associated to each point in the grid are grouped together and averaged, leading to a new representation $\widetilde{\mathbf{P}}$ of the point cloud. 
This new representation is then fed to an encoder-decoder module that is responsible for segmenting $\widetilde{\mathbf{P}}$.
A UNet-based architecture [] is used with 3D sparse convolutional and 3D sparse transposed convolutional layers, where the goal is to segment the foreground points, i.e., points belonging to the ground-truth bounding boxes, from all the other points.
Concurrently, an additional module is designed for learning the intra-object part information.
Given the points $\widetilde{\mathbf{p}}_{f,j}$ with $f = 1, \ldots, F_j$, where $F_j$ denotes the number of foreground points inside the ground-truth bounding box $\mathbf{b}_j$, the intra-object part location for each foreground point is then defined as 
\begin{equation}
	\widetilde{\mathbf{p}}_{f,j}^{(\text{part})} = \left[\dfrac{\Delta \widetilde{p}_{f,j,x}}{w_j} + .5, \dfrac{\Delta \widetilde{p}_{f,j,y}}{\ell_j} + .5, \dfrac{\Delta \widetilde{p}_{f,j,z}}{h_j} + .5\right]^{\mathrm{T}} , 
\end{equation}
where 
\begin{equation}
\left[
\begin{matrix}
\Delta \widetilde{p}_{f,j,x} \\
\Delta \widetilde{p}_{f,j,y} \\
\Delta \widetilde{p}_{f,j,z}
\end{matrix} \right] = \left[ 
\begin{matrix}
\widetilde{p}_{f,j,x} - u_{x,j}^{(\text{B})} \\
\widetilde{p}_{f,j,y} - u_{y,j}^{(\text{B})} \\
\widetilde{p}_{f,j,z} - u_{z,j}^{(\text{B})} \\
\end{matrix}
\right]^{\mathrm{T}} \left[
\begin{matrix}
\cos{\gamma_j} & \sin{\gamma_j} & 0 \\ 
-\sin{\gamma_j} & \cos{\gamma_j} & 0 \\
0 & 0 & 1  
\\
\end{matrix} \right] \, .
\end{equation}
Then, a region proposal network is appended for generating the 3D proposals, using the same strategy of PointiPillars.
Specifically, prior boxes are generated using a fixed grid and only the ones having a sufficiently high overlap with the ground-truths are retained for further refinement.


Once the proposal have been generated, a second network is responsible for improving the detection accuracy.
This module takes as input the intra-object part locations estimated before together with the proposals and the associated features learned and refines the estimated bounding boxes. 
At first, the points falling within each proposal are transformed into a canonical coordinate system where the $x$ and $y$ axis are approximately parallel to the ground plane, while the $z$ is the same as the input point cloud. 
This allows to reduce the impact of different rotation angles and locations of the proposals, leading to a better bounding box regression.
Then, a Region of Interest (RoI)-aware pooling strategy is used to aggregate the features produced during the previous stage.
Specifically, given a proposal $\widetilde{\mathbf{b}}_j$ and the associated canonical foreground points $\widetilde{\mathbf{P}}_{c,j}$, the features $\mathcal{F}_{1}$ containing the segmentation scores and the intra-object part locations are pooled according to 
\begin{equation}
\mathcal{Q}^{(\text{part})} = \text{RoIAwareAvgPool}(\widetilde{\mathbf{P}}_{c,j},\mathcal{F}_1,\widetilde{\mathbf{b}}_j) 
\end{equation}
where $\text{RoIAwareAvgPool}(\cdot)$ is defined as in~\cite{parta2}. 
Similarly, the features $\mathcal{F}_{2}$ extracted from the segmentation process associated with $\widetilde{\mathbf{P}}_{c,j}$ are pooled as  
\begin{equation}
\mathcal{Q}^{(\text{sem})} = \text{RoIAwareMaxPool}(\widetilde{\mathbf{P}}_{c,j},\mathcal{F}_2,\widetilde{\mathbf{b}}_j) 
\end{equation} 
where $\text{RoIAwareMaxPool}(\cdot)$ is defined as in~\cite{parta2}.
After the pooling process, $\mathcal{Q}^{(\text{part})}$ is fed to a submanifold sparse convolutional layer and it is concatenated with $\mathcal{Q}^{(\text{sem})}$ to produce the  features $\mathcal{Q}^{(\text{tot})}$.
$\mathcal{Q}^{(\text{tot})}$ is then fed to sparse convolutional layers to obtain the final representation which is used by two separate branches for bounding box regression and classification.
For obtaining better estimation performances, a 3D-IoU guided scoring mechanism is used~\cite{parta2}. 

Part-$\text{A}^2$ is trained in an end-to-end manner exploiting the following losses.
The segmentation process uses the focal loss $\mathcal{L}_{seg}$ to learn the segmentation masks with the same parameters as in \eqref{eq:focal_loss}, where $p$ now is the probability of a foreground point.
On the other hand, the loss used for leaning the intra-object part classification is the binary cross-entropy
\begin{equation}
\mathcal{L}_{part} = -\widetilde{\mathbf{p}}_{f,j}^{(\text{part})} \log{\widehat{\mathbf{p}}_{f,j}^{(\text{part})}} - (1-\widetilde{\mathbf{p}}_{f,j}^{(\text{part})}) \log(1 - \widehat{\mathbf{p}}_{f,j}^{(\text{part})})
\label{eq:loss_part}
\end{equation}
where $\widehat{\mathbf{m}}_{f,j}^{(\text{part})}$ denotes the predicted intra-object part location. 
The overall loss function used for optimizing the first part of the model is 
\begin{equation}
\mathcal{L}_{\text{first}} = \mathcal{L}_{\text{seg}} +\dfrac{1}{N_f} \mathcal{L}_{\text{part}} + \lambda_{loc}\dfrac{1}{N_{pos}}\mathcal{L}_{\text{loc}}
\end{equation}
where $N_f$ is the number of foreground points, $N_{pos}$ the number of positive prior boxes, $\lambda_{loc} = 2$ and $\mathcal{L}_{\text{loc}}$ is the same loss function defined in \eqref{eq:loc_loss_pointpillars}.
The second part of the \ac{nn} is trained by minimizing the following loss
\begin{equation}
\mathcal{L}_{\text{second}} = \mathcal{L}_{\text{score}} + \dfrac{1}{T_{\text{pos}}} \mathcal{L}_{\text{refine}} \, , 
\end{equation}
where $\mathcal{L}_{score}$ is a binary cross-entropy loss, defined as in \eqref{eq:loss_part}, which is used for the 3D-IoU guided scoring mechanism, while 
\begin{equation}
\mathcal{L}_{\text{refine}} = \mathcal{L}_{\text{loc}} + \mathcal{L}_{\text{corner}}
\end{equation}
where $\mathcal{L}_{\text{loc}}$ is the same loss as in \eqref{eq:loc_loss_pointpillars} but with $\Delta \gamma = \hat{\gamma}_j - \gamma_j$, and 
\begin{equation}
\mathcal{L}_{\text{corner}} = \mathrm{S_{L1}}(\|\mathbf{z}_{j}^{(B)} - \hat{\mathbf{z}}_{j}^{(B)}  \|)
\end{equation}
where $\mathbf{z}_{j}^{(B)} = [z_{j,1}^{(B)}, \ldots z_{j,8}^{(B)}]$ and $\hat{\mathbf{z}}_{j}^{(B)} = [\hat{z}_{j,1}^{(B)}, \ldots \hat{z}_{j,8}^{(B)}]$ are the corners of the ground-truth and predicted bounding boxes. 
Finally, the overall loss used for optimizing the trainable parameters of Part-$\text{A}^2$ is
\begin{equation}
\mathcal{L}_{\text{total}} = \mathcal{L}_{\text{first}} + \mathcal{L}_{\text{second}}
\end{equation} 


Both the \ac{dnn} detectors are trained in a centralized manner and then deployed at vehicles. In this way, each vehicle $i$ can estimate the bounding boxes from the point cloud  $\mathbf{P}_{v,t}$ and obtain the corresponding sets $\boldsymbol{\rho}_{v,t}^{\text{(O)}}$ and $\mathbf{z}_{v,t}^{\text{(O)}}$.


==> sections/NumericalResults.tex <==
% \section{3D object detection results}
% \label{sec:numerical_results}

% \begin{table*}[!t]
% %\vspace{-3mm}
% \renewcommand{\arraystretch}{1.3}
% \setlength{\tabcolsep}{4pt}
% \caption{3D object detection performance analysis}
% \label{tab:map}
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%     \hline
%      \multirow{3}{*}{\textbf{Detector}}  & \multicolumn{6}{c|}{\textbf{$\text{AP}_{\text{BEV}}$}} &  \multicolumn{6}{c|}{\textbf{$\text{AP}_{\text{3D}}$}} \\ \cline{2-13}
%      & \multicolumn{3}{c|}{$L = 11$} & \multicolumn{3}{c|}{$L = 40$} & \multicolumn{3}{c|}{$L = 11$} & 
%      \multicolumn{3}{c|}{$L = 40$} \\  \cline{2-13}
%      & $\varepsilon = 0.25$ & $\varepsilon = 0.50$ & $\varepsilon = 0.70$ & $\varepsilon = 0.25$ & $\varepsilon = 0.50$ & $\varepsilon = 0.70$ & $\varepsilon = 0.25$ & $\varepsilon = 0.50$ & $\varepsilon = 0.70$ & $\varepsilon = 0.25$ & $\varepsilon = 0.50$ & $\varepsilon = 0.70$ \\ \hline
%      PointPillars & 93.51 & 93.49 & 93.20 & 96.15 & 96.12 & 95.44 & 93.51 & 93.49 & 88.54 & 96.15 & 96.12 & 90.78 \\
%      PointRCNN & 88.72 & 88.72 & 88.48 & 91.38 & 91.38 & 91.14 & 88.71 & 88.58 & 74.64 & 91.38 & 91.15 & 75.18\\ \hline
%     \end{tabular}
% \end{table*}

% \textcolor{red}{aggiungi dettagli sul training, numero di epoche, learning rate, scheduling, data augmentation ecc...
% Aggiungi come vengono generate le traiettorie dei veicoli e che partono da fermi -> specifica che il testing è fatto sulla stessa mappa ma le traiettoria sono differenti da quelle della validazione}


% \textcolor{green}{In this section, we presents the numerical results for the proposed \ac{dnn-icp} method in two challenging simulated road scenarios.
% Sec.~\ref{subsec:obj_detection_results} show the detection performances of the selected LiDAR-based 3D object detection methods, while Sec.~\ref{subsec:results_coop_loc} focuses on the characterization of the overall cooperative localization scheme.   }

% %This section presents the assessment of the proposed \ac{dnn-icp} method in a simulated road scenario. 
% %Sec.~\ref{subsec:obj_detection_results} only considers the detection performance of the PointPillars model, while Sec.~\ref{subsec:results_coop_loc} provides a comprehensive characterization of the achievable localization performance.

% %Cooperative positioning systems enable the fusion of location-related information across interconnected agents to improve the accuracy of the agents’ localization. In this section, we discuss the application of this approach to V2X-networked vehicles in a urban mobility usecase, where implicit cooperative positioning \cite{icp} is used to augment not only the vehicle positioning but also the detection and tracking of objects sensed sensed by the vehicles in the driving environment by fusing data from on-board GPS and imaging sensors with nearby vehicles via V2X links. The example shows the benefits of the cooperative approach over conventional ego-vehicle solutions that rely only on on-board sensors to obtain the location and mapping information. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/carla_town02.png}
%     \caption{Top-view of the Town02 simulation scenario from Carla}
%     \label{fig:carla_map_tonw02}
% \end{figure}



% \subsection{LiDAR-based object detection}
% \label{subsec:obj_detection_results}




% \textcolor{green}{This section focuses on the evaluation of the detection performances of the PointPillars and PointRCNN methods.
% In particular, we are interested in their ability to correctly estimate the bounding boxes of the poles from the LiDAR point clouds to characterize the covariance matrix $\mathbf{R}_{i,k,t}^{(\text{DNN})}$ to be employed in the localization scheme detailed in Sec.~\ref{subsec:coop_LiDAR_localization}.
% For this reason, this analysis assumes the vehicle position to be exactly known.
% }
% %This section focuses on the evaluation of the detection performances of the PointPillars and PointRCNN models 

% \textcolor{green}{For training the 3D object detectors, we generated a synthetic dataset from CARLA~\cite{pmlr-v78-dosovitskiy17a}, an advanced autonomous driving simulator that allows flexible configuration of realistic vehicular layouts and sensor specifications.
% The dataset is collected in the urban map \textit{Town02} of CARLA, that spans roughly a $200\times 200$ $\text{m}^{2}$ area, where a single LiDAR-equipped vehicle moves in the environment for 5000 timestamps sampled at $T_s=0.2$ s.
% The considered map is depicted in Fig.~\ref{fig:carla_map_tonw02} where several buildings, trees and road intersections can be appreciated.}

% The LiDAR sensor is placed on the roof of the vehicle and is configured to have 64 planes covering an elevation angle between $-25$° and $15$°, a sensing range of $70$ m and to output 1 million point clouds per second, on average, with a $\pm 2$~cm accuracy. 
% For a more realistic simulation, we randomly remove $20\%$ of the points for each captured frame. 
% The ground truth data consists of 3D bounding boxes physically enclosing the poles.
% We remove from the ground-truths any box that has less than 10 points inside. 
% %A training example is provided in Fig.~\ref{fig:train_ex} where the ground-truth bounding boxes are highlighted with green lines.  
% The performances of the object detector are evaluated over an held-out portion of the dataset composed by $1000$ examples, while the remaining $4000$ ones are used for training. 
% \textcolor{green}{Both detectors are trained using data augmentation strategies to improve their performances and generalize to new, unseen scenarios. 
% In particular, we create a database containing all ground-truth boxes that contains at least 10 points inside and their associated point clouds from the training set and apply ground-truth sampling: for every point cloud we add at most $5$ ground-truth boxes and the corresponding points in random positions of the point cloud to enrich the training examples.
% The point cloud is further augmented by applying a random rotation inside the interval $[-\pi/2, \pi/2]$, random scaling between $95\%$-$105\%$ of the original point cloud, and random horizontal flip with respect to the $z$-axis. 
% PointPillars is trained for $80$ epochs with the Adam \cite{adam} optimizer with an initial learning rate of $0.0003$, momentum parameters $\{0.95, 0.85\}$, and a weight decay factor of $0.001$.
% Similarly, PointRCNN is trained for $80$ epochs with an initial learning rate of $0.0125$ and with other parameters the same as PointPillars. 
% For both models, we apply a cosine annealing scheduling strategy~\cite{cosine_annealing}  without warm restarts where the learning rate increases up to 10 times the initial learning rate until the 40th epoch and then decreases to its initial value. 
% }
% As an example, Fig.~\ref{fig:aggregated_point_cloud} shows the (aggregated) LiDAR point clouds gathered by 20 vehicles (red boxes) and the poles (green boxes) in the area, during a simulation frame.

% \textcolor{green}{As performance metric we use the \ac{ap} \cite{pascal_voc} which is evaluated as the average of the area under the interpolated precision/recall curve over a set of recall levels.
% For object detection tasks, the \ac{ap} requires the computation of the \ac{iou} to discern positive and negative predictions.
% Given a pair of $\{\mathbf{b}_j, \widehat{\mathbf{b}}_j \}$ of ground-truth and predicted bounding boxes, the \ac{iou} is the ratio of the volume of the intersection and the volume of the union between $\mathbf{b}_{j}$ and $\widehat{\mathbf{b}}_{j}$.
% Thus, it is
% \begin{equation}
%     \text{IoU}(\mathbf{b}_j, \widehat{\mathbf{b}}_j) = \dfrac{\text{volume}(\mathbf{b}_j \cap \widehat{\mathbf{b}}_j)}{\text{volume}(\mathbf{b}_j \cup \widehat{\mathbf{b}}_j)}
% \end{equation}
% and $\widehat{\mathbf{b}}_{j} $ is deemed as positive if the \ac{iou} is greater than a threshold $\varepsilon$.
% Then, the precision can be evaluated as the ratio between the number of correct positive predictions and the total number of positive predictions. 
% Similarly, the recall is the ratio between the number of correct positive predictions and the total number of ground-truths.
% Given $L$ equally-spaced recall levels in the interval $[0 \, 1]$, the \ac{ap} is computed as
% \begin{equation}
%     \text{AP} = \sum_{\ell = 1}^{L} e_{irp}(r_{k+1})\left[r_{k+1} - r_{k}\right]
% \end{equation}
% where
% \begin{equation}
%     e_{irp}(r) = \underset{\tilde{r} > r}{\text{max}} \,  e(\tilde{r})
% \end{equation}
% is the interpolated version of the precision-recall curve where the maximum precision value is considered for which the corresponding recall value exceeds $r$. 
% In the following we use $L=11$ and $L = 40$ as recently suggested in \cite{map_recall_levels}.}
% As an additional performance metric, we evaluate the localization error of the predicted bounding boxes with respect to the ground-truths, neglecting any false positive.
% In particular, we  consider the centroid of the bounding box to assess how accurate and precise are the predictions with respect to the ground-truths.
% We use the \ac{cdf} of the location error $\mathbf{e}_{b} = \| \widehat{\mathbf{u}}_{j}^{(\text{B})} - \mathbf{\mathbf{u}}_{j}^{(\text{B})} \|$ between the true bounding box $\mathbf{b}_{j}$ and the predicted one $\widehat{\mathbf{b}}_{j}$ and compute the \ac{cep} at $9$5\% confidence.
% Both performance metrics are evaluated on the validation dataset. 

% \begin{figure}[!t]
% \subfloat[\label{fig:preds_pointpillars}]{
% \includegraphics[width=0.95\columnwidth]{images/preds_pointpillars.pdf}
% }

% \vspace{-3mm}
% \subfloat[\label{fig:preds_pointrcnn}]{
% \includegraphics[width=0.95\columnwidth]{images/preds_pointrcnn.pdf}
% }

% \vspace{-3mm}
% \subfloat[\label{fig:true_boxes}]{
% \includegraphics[width=0.95\columnwidth]{images/true_boxes.pdf}
% }
%     \caption{Example of the output obtained by the 3D object detectors: (a) PointPillars, (b) PointRCNN, (c) Ground-truths. }
%         \label{fig:qualitative_results_detection}
% \end{figure}


% \begin{figure}[!t]
% \centering
%     \includegraphics[width=\linewidth]{images/bbox_location_cdf.pdf}
%     \caption{CDF of bounding box location error $\mathbf{e}_{b}$ using PointPillars and PointRCNN.}
%    \vspace{-3mm}
%     \label{fig:bbox_location_cdf}
% \end{figure}


% \textcolor{green}{Table~\ref{tab:map} reports the \ac{ap} for the two detectors considering \ac{iou} thresholds $\varepsilon = \{0.25, 0.50,0.70\}$ and recall levels $L = \{11, 40\}$.
% The \ac{ap} is evaluated over the \ac{bev} projection, denoted as $\text{AP}_{\text{BEV}}$, which projects the predictions onto the $x$-$y$ plane and in the 3D space, referred to as $\text{AP}_{\text{3D}}$.}

% %Table~\ref{tab:map} reports the results of the validation considering an \ac{iou} threshold of $\varepsilon = \{0.25, 0.50,0.70\}$. The \ac{ap} is evaluated using the \ac{bev} projection, denoted as $\text{AP}_{\text{BEV}}$, which projects the predictions onto the $x$-$y$ plane and in the 3D space, referred to as $\text{AP}_{\text{3D}}$. The detection results show that the \ac{nn} is able to precisely recognize poles in the driving environment.
% As expected, the $\text{AP}_{\text{BEV}}$ is superior compared to $\text{AP}_{\text{3D}}$ since it does not consider the predictions over the $z$-axis. 
% Interestingly, the $\text{AP}_{\text{BEV}}$ almost coincides with $\text{AP}_{\text{AP}}$ when $\varepsilon = 0.25$, while for greater \ac{iou} values the gap between the two increases.



% To further characterize the performance of PointPillars,  in Fig.~\ref{fig:bbox_location_cdf} we report the \ac{cdf} of the location error  $\mathbf{e}_{b}$. The results confirm the high accuracy feature detection of the \ac{dnn} model.
% Indeed, the location error over the bounding box center is less than $5$~cm in 95\% of the cases.
% %and less than $20$~cm for all predicted bounding boxes. 

% %\begin{figure}
% %     \centering
% %     %\vspace{2mm}
% %     \includegraphics[width=\columnwidth,keepaspectratio]{images/cooprative_point_cloud.pdf}
%      %\vspace{-7mm}
% %     \caption{Aggregated point cloud data acquired by 20 vehicles (red bounding boxes) and  72 poles (green bounding boxes).}
% %     \label{fig:aggregated_point_cloud}
% %\end{figure}

% %Given the pair $\{\mathbf{b}_j, \widehat{\mathbf{b}}_j \}$ of ground-truth and predicted bounding boxes we evaluate $\mathbf{e}_{b} = \| \widehat{\mathbf{u}}_{j}^{(\text{B})} - \mathbf{\mathbf{u}}_{j}^{(\text{B})} \|$ and  

% %\begin{equation}
    
% %\end{equation}
% %We employ a synthetic dataset extracted from CARLA software \cite{pmlr-v78-dosovitskiy17a} to evaluate the performances of the 3D object detector in locating the features.







% \begin{figure}[!t]
%      \centering

%      \includegraphics[width=0.75\columnwidth,keepaspectratio]{images/snapshot_v2.pdf}
     
%      \caption{Carla Simulator: Snapshot of CARLA simulator with vehicles (red circles), 
%      poles (green cubes) and LiDAR-based detections (black solid line).}
%      \label{fig:snapshot}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/missed_detections_comparison_town02.pdf}
%     \caption{Analysis of the missed detection percentages varying the LiDAR sensing range for PointPillars and PointRCNN}
%     \label{fig:missed_detections_town02}
% \end{figure}

% \begin{figure}[!t]
% \subfloat[\label{fig:fp_map_pointpillars_town02}]{
% \includegraphics[width=0.95\columnwidth]{images/fp_pointpillars_town02.pdf}
% }

% \vspace{-3mm}
% \subfloat[\label{fig:fp_map_pointrcnn_town02}]{
% \includegraphics[width=0.95\columnwidth]{images/fp_pointrcnn_town02.pdf}
% }
%     \caption{Comparison of the spatial distribution of the false positives predicted by (a) PointPillars, (b) PointRCNN.}
%     \label{fig:my_label}
% \end{figure}

% \begin{table}[!t]
% \renewcommand{\arraystretch}{1.3}
% \setlength{\tabcolsep}{4pt}
% \caption{Detection Performances Analysis in Town02}
% \label{tab:my_label}
%     \centering
%     \begin{tabular}{|c|c|c|c|}
%     \hline
%        \multirow{2}{*}{\textbf{Method}}  & \textbf{Correct detections} & \textbf{Missed detections} & \textbf{False positives} \\
%          & [\%] & [\%] & [\%] \\ \hline
%          PointPillars & 89.94 & 10.06 & 23.67 \\
%          PointRCNN & 83.97 & 16.03 & 27.52 \\ \hline
%     \end{tabular}
% \end{table}

% \subsection{Cooperative localization}
% \label{subsec:results_coop_loc}

% \textcolor{red}{Aggiungi risultati mappa per RMSE targets, aggiungi mappa per false positives and missed detections.}

% \textcolor{red}{Aggiungi risultati nuovo scenario}


% % \begin{figure*}
% % \centering
% % \subfloat[\label{fig:snapshot}]{\includegraphics[width=0.75\columnwidth,keepaspectratio]{images/scenario.pdf}}
% % \hspace{18mm}
% % \subfloat[\label{fig:rmse_map_gps}]{
% % \includegraphics[width=0.95\columnwidth]{images/rmse_gps_map.pdf}
% % }

% % \subfloat[\label{fig:rmse_map_icp_dl}]{
% % \includegraphics[width=0.95\columnwidth]{images/rmse_icp_dl.pdf}
% % }
% % \subfloat[\label{fig:rmse_map_icp_LiDAR}]{
% % \includegraphics[width=0.95\columnwidth]{images/rmse_icp_LiDAR.pdf}
% % }

% % \caption{Cooperative localization scenario and performance. a) snapshot of CARLA simulator with vehicles (black circles), poles (red triangles) and LiDAR-based detections (black solid line).
% % Root Mean Square Error (RMSE) of vehicle's position over the whole simulation map for (b) ego-vehicle approach, (c) cooperative solution with PointPillars predictions, (d) cooperative solution with all objects visible within the LiDAR sensing range. Results are averaged over all vehicles.}
% % \label{fig:results_comparison}
% % \end{figure*}






% The cooperative localization scheme is evaluated in the urban scenario \textit{Town02} of CARLA, with twenty vehicles moving in the area.
% %and are equipped with a \ac{gnss} unit for positioning purposes. They also have a LiDAR sensor configured as in Sec.~\ref{subsec:obj_detection_results} to detect poles.
% The on-board \ac{gnss} receiver provides position and velocity information of the vehicles with accuracy (constant all over the space) ruled by $\mathbf{R}_{i,t}^{(\text{GNSS})} = \text{blkdiag}(\sigma_{p}^{\text{(V)}^2} \mathbf{I}_{2} , \sigma_{v}^{\text{(V)}^2} \mathbf{I}_{2})$, with $\sigma_p^{(V)} = 5$ m and $\sigma_v^{(V)} = 0.45$ m/s, respectively. 
% The covariance associated to the LiDAR-based sensing  is set to $\mathbf{R}_{i,k,t}^{(\text{DNN})} = \sigma_{p}^{{\text{(DNN)}^2}} \mathbf{I}_{2}$ with $\sigma_{p}^{(\text{DNN})} = 0.05$ m, in accordance with the analysis in Sec.~\ref{subsec:obj_detection_results}. 
% Calibration of the vehicle motion model \eqref{eq:motion_model} on the CARLA data leads to $\mathbf{Q}_{i,t-1}^{(\text{V})} = \text{diag}(\sigma_{vi,x}^{\text{(\text{V})}^2}, \sigma_{vi,y}^{\text{(\text{V})}^2})$, with $\sigma_{vi,x}^{(\text{V})} = \sigma_{vi,y}^{(\text{V})} = 0.5$ m/${\text{s}^2}$.
% The overall duration of the simulation is $300$ s with a time interval between adjacent frames of $T_s = 0.2$ s.
% Fig.~\ref{fig:snapshot} provides a view of the scenario for a single frame, where vehicles are denoted by red dots and poles by green cubes, while the solid black lines show the detections made by vehicles.
% %, resulting in $1500$ snapshots of the scenario. 

% The performance analysis focuses on the comparison of the following positioning solutions:
% \begin{itemize}
%     \item The proposed \ac{dnn-icp} method where cooperative \ac{kf} is performed using as passive objects the poles detected by PointPillars at each vehicle within range $R_s$;
%     \item An oracle \ac{dnn-icp} (O-DNN-ICP) with perfect LiDAR sensing of all objects within $R_s$, regardless of visibility conditions;
%     \item A conventional tracking system based on a \ac{kf} that integrates position and velocity information provided by the on-board \ac{gnss} unit, referred to as GNSS-KF;
% \end{itemize}
% The difference between \ac{dnn-icp} and O-DNN-ICP is that, on average, \ac{dnn-icp} misses the detections of  9.6\% of detectable objects. The performances are evaluated over $N_{\text{MC}} = 100$ Monte Carlo simulation by computing the \ac{rmse} of vehicle position.
% % The performances are evaluated over $N_{\text{MC}} = 100$ Monte Carlo simulation by computing the location \ac{rmse} of the vehicles defined as $\text{RMSE}_t = (\sum_{n=1}^{N_{\text{MC}}} \|\mathbf{u}_{i,t}^{(\text{V})} - \widehat{\mathbf{u}}_{i,t}^{(\text{V})}\|^2 / N_{\text{MC}})^{0.5}$.
% %where $\mathbf{u}_{i,t}^{(\text{V})}$ and $\widehat{\mathbf{u}}_{i,t}^{(\text{V})}$ are the true and estimated vehicle positions at time $t$.

% %We consider a urban scenario simulated in CARLA \cite{pmlr-v78-dosovitskiy17a}, an advanced autonomous driving simulator that allows flexible configurations of vehicular layouts and sensor specifications. Twenty vehicles move in the map Town02 that spans roughly a 200x200 m area and are equipped with a GPS for positioning purposes along with a LiDAR sensor to detect vulnerable road users, i.e., pedestrians, as well as static features present in the environment, such as traffic signs, traffic lights and poles. All LiDAR sensors are placed on the vehicles’ roof and configured to have 64 planes covering an elevation angle between -25° and 15°, a maximum sensing range of 70 m and to output 1 million point clouds per second, on average, each with a ± 2 cm accuracy. These values reflect the technical parameters characterizing most commercially available LiDAR systems.

% %The on-board GPS provides the position and velocity of the vehicle with a 5 m and 0.45 m/s accuracy, respectively. The cooperative positioning scheme relies on a centralized processing unit to collect data generated by the on-board LiDAR at the vehicles regarding the location of passive static targets, namely poles, to be fused for positioning augmentation. In particular, poles are assumed to be detected if their position fall within the field of view of the LiDAR sensor. If so, they can be precisely localized relatively to the moving vehicle with a 0.1 m accuracy. To ease the implementation, we assume that the association between LiDAR measurements and passive targets is perfectly know at all time instants. On the other hand, the ego-vehicle positioning solution uses an Extended Kalman Filter (EKF) to track the vehicles state, i.e., position and velocity, over time exploiting only the GPS measurements. 
% %The overall duration of the simulation is 300 s with a time interval between adjacent frames of 0.2 s, resulting in 1500 snapshots of the scenario. An example of such a snapshot is provided in Fig. 1, where vehicles are denoted by black dots and poles by red triangles, while the solid black lines show the detections made by vehicles.



% \begin{figure*}
% \centering
% \subfloat[\label{fig:rmse_map_gps}]{
% \includegraphics[width=0.85\columnwidth]{images/rmse_gps_map.pdf}
% }
% \subfloat[\label{fig:rmse_map_icp_dl}]{
% \includegraphics[width=0.85\columnwidth]{images/rmse_icp_dl.pdf}
% }

% \vspace{-3mm}
% \subfloat[\label{fig:rmse_map_icp_LiDAR}]{
% \includegraphics[width=0.85\columnwidth]{images/rmse_icp_LiDAR.pdf}
% }
% \subfloat[\label{fig:rmse_map_icp_pointrcnn}]{
% \includegraphics[width=0.85\columnwidth]{images/rmse_icp_pointrcnn.pdf}
% }
% %\subfloat[\label{fig:icp_bound}]{
% %\includegraphics[width=0.65\columnwidth]{images/icp_bound.pdf}
% %}

% \caption{Spatial RMSE of vehicle positions over the simulation map.  (a) GNSS-KF. (b) \ac{dnn-icp}. (c) O-DNN-ICP (d) \ac{dnn-icp} PointRCNN}
% \label{fig:results_comparison}
% \vspace{-4mm}

% \end{figure*}

% \begin{table}[!t]
% \renewcommand{\arraystretch}{1.3}
% \setlength{\tabcolsep}{4pt}
%     \caption{Analysis of cooperative localization performance against LiDAR sensing range}
%     \label{tab:my_label}
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%      \multirow{2}{*}{Method} & \multirow{2}{*}{$R_s$} & \multicolumn{2}{c|}{Vehicles} & \multicolumn{2}{c|}{Targets}\\ \cline{3-6}
%      & & RMSE & CEP95 & RMSE & CEP95 \\ \hline 
%      \multirow{6}{*}{DNN-ICP  PointPillars}  & 70 & - & - & - & -\\
%      & 60 & - & - & - & -\\
%      & 50 & - & - & - & -\\
%      & 40 & - & - & - & -\\
%      & 30 & - & - & - & -\\
%      & 20 & - & - & - & -\\ \hline 
%      \multirow{6}{*}{DNN-ICP  PointRCNN}  & 70 & - & - & - & -\\
%      & 60 & - & - & - & -\\
%      & 50 & - & - & - & -\\
%      & 40 & - & - & - & -\\
%      & 30 & - & - & - & -\\
%      & 20 & - & - & - & -\\ \hline 
%     \multirow{6}{*}{O-DNN-ICP}  & 70 & - & - & - & -\\
%      & 60 & - & - & - & -\\
%      & 50 & - & - & - & -\\
%      & 40 & - & - & - & -\\
%      & 30 & - & - & - & -\\
%      & 20 & - & - & - & -\\ \hline   
%     \end{tabular}
% \end{table}

% Fig.~\ref{fig:results_comparison} reports the results of the comparison, highlighting the spatial \ac{rmse} over the simulation map obtained by the stand-alone GNSS-KF tracking scheme (Fig.~\ref{fig:rmse_map_gps}), the proposed \ac{dnn-icp} (Fig.~\ref{fig:rmse_map_icp_dl}) and the O-DNN-ICP (Fig.~\ref{fig:rmse_map_icp_LiDAR}).
% The results show that the cooperative \ac{icp} methods outperform the ego GNSS-KF filtering solution by a large margin, for nearly all positions. 
% %Indeed, the RMSE of the cooperative approaches is largely reduced compared to the one obtained by the GNSS-KF for, nearly, all positions of the map.
% Still, some locations can be spot where the improvement brought by the cooperation is marginal, e.g., at the center of the leftmost vertical road. This is related to the fact that some areas may be less frequently visited by vehicles, resulting in a decreased level of cooperation. %and consequently a higher \ac{rmse}. 
% Thus, the cooperation is beneficial, especially  when a sufficient number of vehicles concurrently observe the same area. 
% %Nevertheless, the results indicate that relying on cooperative schemes is beneficial for increasing localization accuracy, especially when a sufficient number of vehicles concurrently observe the same area. 
% Comparing the two \ac{icp} methods, a negligible performance loss is experienced by \ac{dnn-icp} when compared to O-DNN-ICP (see e.g., the uppermost horizontal road and leftmost vertical road).
% Results indicate that the proposed cooperative strategy can be used to augment \ac{gnss} even when not all features are detected due to poor visibility or for too far objects. This is also confirmed by Fig.~\ref{fig:cdf_comparison}, which shows the \ac{cdf} of the location \ac{rmse} and the \ac{cep} 95\% for the two cooperative methods. \ac{dnn-icp} has comparable performances with respect to \linebreak O-DNN-ICP  even if it misses 9.6\% of detections. The \ac{cep} 95\%  is $31$ cm for \ac{dnn-icp} and $24$ cm for O-DNN-ICP.
% %To further characterize the proposed method and analyze its properties against O-DNN-ICP, we compare in Fig.~\ref{fig:cdf_comparison} the \ac{cdf} of the location \ac{rmse} for the cooperative methods and highlight the \ac{cep} 95\% for both approaches. 
% %We also report the sum of the number of undetected features for all vehicles, i.e., missed detections, for every simulation timestamp in Fig.~\ref{fig:undetected_targets}. This is shown only for \ac{dnn-icp} as O-DNN-ICP assumes to always detect all features for all simulation timestamps. 

% % This shows that a moderate performance loss is experienced by \ac{dnn-icp} compared to O-DNN-ICP allowing some room for an imperfect feature detection process. 
% % Furthermore, not all objects may be relevant for the cooperative scheme as only those jointly sensed by multiple vehicles are considered for positioning enhancement. 

% \begin{figure}[!t]
% %\vspace{-5mm}
%     \centering
%     \includegraphics[width=\linewidth]{images/cdf_comparison.pdf}
%     %\vspace{-7mm}
%     \caption{CDF of vehicle position RMSE for DNN-ICP and O-DNN-ICP.}
%     \label{fig:cdf_comparison}
% \end{figure}


% %\begin{figure}
% %\vspace{-3mm}
% %    \centering
% %    \includegraphics[width=\linewidth]{images/undetected_targets.pdf}
% %    \vspace{-8mm}
% %    \caption{Number of undetected targets vs simulation timestamp for the \ac{dnn-icp} cooperative localization scheme.}
% %    \label{fig:undetected_targets}
% %\end{figure}
